Correctness of Automatic Differentiation via Diffeologies and Categorical Gluing

We present semantic correctness proofs of Automatic Differentiation (AD). We consider a forward-mode AD method on a higher order language with algebraic data types, and we characterise it as the unique structure preserving macro given a choice of derivatives for basic operations. We describe a rich semantics for differentiable programming, based on diffeological spaces. We show that it interprets our language, and we phrase what it means for the AD method to be correct with respect to this semantics. We show that our characterisation of AD gives rise to an elegant semantic proof of its correctness based on a gluing construction on diffeological spaces. We explain how this is, in essence, a logical relations argument. Finally, we sketch how the analysis extends to other AD methods by considering a continuation-based method.

==> beta-eta.tex <==
\[
\begin{array}{l}
\tMatch{\tTriple{\trm_1}{\ldots}{\trm_n}}{\var_1,\ldots,\var_n}{\trm[2]}=
\subst{\trm[2]}{\sfor{\var_1}{\trm_1},\ldots,\sfor{\var_n}{\trm_n}}\\
\subst{\trm[2]}{\sfor{\var[2]}{\trm}}\freeeq{\var_1,\ldots,\var_n}
\tMatch{\trm}{\var_1,\ldots,\var_n}{\subst{\trm[2]}{
    \sfor{\var[2]}{\tTriple{\var_1}{\ldots}{\var_n}}}}\\
(\fun{\var}{\trm})\,\trm[2] = \subst{\trm}{\sfor{\var}{\trm[2]}}\qquad\qquad\qquad\trm \freeeq{\var} \fun{\var}{\trm\,\var}
\end{array}
\]

==> beta-eta2.tex <==
\[
\begin{array}{l}
    \vMatch {\Inj{\Cns_i}{\trm}  }  {
        \Inj{\Cns_1}{\var_1}\To{\trm[2]_1}
\vor \cdots
\vor  \Inj{\Cns_n}{\var_n}\To{\trm[2]_n}
} = \subst{\trm[2]_i}{\sfor{\var_i}{\trm}}\\
\subst{\trm[2]}{\sfor{\var[2]}{\trm}}\freeeq{\var_1,\ldots,\var_n}
\vMatch {\trm}  {
        \Inj{\Cns_1}{\var_1}\To{\subst{\trm[2]}{\sfor{\var[2]}{\Inj{\Cns_1}{\var_1}}}}
\vor \cdots
\vor  \Inj{\Cns_n}{\var_n}\To{\subst{\trm[2]}{\sfor{\var[2]}{\Inj{\Cns_n}{\var_n}}}}
}\\
\lFold{\var_1}{\var_2}{\trm}{\tNil}{\trm[3]} = \trm[3] \\
\lFold{\var_1}{\var_2}{\trm}{\tCons{\trm[2]_1}{\trm[2]_2}}{\trm[3]} =
\subst{\trm}{\sfor{\var_1}{\trm[2]_1},\sfor{\var_2}
{\lFold{\var_1}{\var_2}{\trm}{\trm[2]_2}{\trm[3]}}}
 \\
u= \subst{\trm[2]}{\sfor{\var[2]}{\tNil}} ,
\subst{\trm[3]}{\sfor{\var_2}{\trm[2]}}
=\subst{\trm[2]}{\sfor{\var[2]}{\tCons{\var_1}{\var[2]}}}
\Rightarrow
 \subst{\trm[2]}{\sfor{\var[2]}{\trm}} \freeeq{\var_1,\var_2}
\lFold{\var_1}{\var_2}{\trm[3]}{\trm}{u}
\end{array}
\]


==> introduction.tex <==
\section{Introduction}\label{sec:introduction}

\subsubsection{Why differential algorithms matter.}
Many of the most important advances in machine learning and computational statistics in recent decades rely on the use of
\emph{differential algorithms}, algorithms computing derivatives of mathematical functions.
Indeed, many problems in these fields either reduce to the two fundamental computational tasks of
\begin{tightitemize}
  \item \emph{optimization}, to find an optimum value of an objective function, like a maximum likelihood estimate,
  \item \emph{(Monte-Carlo) integration}, to calculate an average (or integral, or expectation value) of some quantity with respect to some potentially unnormalised probability distribution.
\end{tightitemize}
These tasks tend to be referred to collectively as \emph{inference} tasks, as they subsume both maximum likelihood estimation and Bayesian inference.
When working on high dimensional spaces -- i.e. for models with a lot of parameters -- derivative information is a crucial heuristic to help solve these tasks in practice:
\begin{tightitemize}
  \item Optimization problems have very successfully been tackled using methods like (stochastic) gradient descent (SGD) \cite{robbins1951stochastic,kiefer1952stochastic}, SGD with momentum \cite{qian1999momentum}, Adam \cite{kingma2014adam}, AdaGrad \cite{duchi2011adaptive}, L-BFGS \cite{liu1989limited} which rely on first order derivatives, or even using methods which rely on higher order ones like the Newton's method.
  \item More surprisingly, Monte-Carlo integration problems in high dimension have also most successfully been solved using methods which  rely on derivatives like Hamiltonian Monte-Carlo \cite{neal2011mcmc}, the No-U-Turn Sampler \cite{hoffman2014no}, and various differentiation-based variational inference methods like Automatic-Differentiation Variational Inference \cite{kucukelbir2017automatic}.
  Somewhat paradoxically, it can help to differentiate a function in order to integrate it.
\end{tightitemize}
\vspace{-10pt}
\subsubsection{Algorithmic differentiation and differential programming.}
The ubiquity of the need to calculate derivatives of functions efficiently has led to three classes of techniques for calculating such derivatives:
\begin{tightenumerate}
  \item[1)\hspace{-1pt}] the method of \emph{finite differences} -- approximating the derivative of a function $f$ at $a$ as $\lim_{\Delta\to 0}\frac{f(a+\Delta) - f(a)}{\Delta}$;
  \item[2)\hspace{-1pt}] \emph{symbolic differentiation} -- using pre-programmed computer algebra rules to calculate derivatives symbolically, for example using the algebraic identity that the derivative of $x\mapsto x^n$ is $x\mapsto n \cdot x^{n-1}$;
  \item[3)\hspace{-1pt}] \emph{automatic differentiation (AD)} -- using the chain rule for differentiation to calculate the derivative of composite programs in terms of the derivatives of parts, for example calculating the derivative of $g;f$ at $a$ as $\frac{\dif f}{\dif y}(g(a))\cdot \frac{\dif g}{\dif x}(a)$.
\end{tightenumerate}
While method 1) is an indispensable means for testing the correctness of the implementation of methods 2) and 3), it can typically not compete in terms of efficiency and numerical stability.
State-of-the-art systems often rely on a combination of methods 2) and 3): (recursively) using a symbolic derivative when a suitable rule is available and otherwise backing off to applying the chain rule.
This combination is often -- confusingly -- also referred to as automatic differentiation.
Depending on the system, the differentiation can be implemented either by explicitly applying a source-code transformation to the original code or by interpreting the code at non-standard types through operator overloading, arguably defining a similar source-code transformation rather more implicitly.


Because of the importance of differentiation for inference, modelling languages and libraries for machine learning and computational statistics like the Stan language and TensorFlow consist exclusively of differentiable language constructs.
That is, they are examples of \emph{differential programming languages}.
With increasing modelling needs in these fields, there is a growing demand for expressive and efficient differential programming languages \cite{olah2015neural,lecun2018deep}.
The demand for efficiency has led to an increasing complexity in the techniques for implementing automatic differentiation: forward (fwd) mode AD \cite{wengert1964simple}, reverse (rev) mode AD \cite{linnainmaa1970representation,speelpenning1980compiling,rumelhart1988learning}, higher order AD through nesting \cite{griewank2008evaluating}, (currently very experimental) jet-based higher order AD \cite{betancourt2018geometric}.
The relative efficiency of these techniques depends on the (dimensions of the) particular program being differentiated; thus, they are all of interest.
For example, for first order AD, one would typically choose fwd mode for programs with outputs of (much) higher dimension than the input and rev mode otherwise.
The demand for expressiveness leads to the introduction of rich language features into differential languages like higher order functions, tuples, variants, iteration, recursion, inductive types, recursive types and  types corresponding to manifolds.
Both of these aspects of efficiency and expressiveness add to the complexity of differential programming systems and make it a non-trivial task to implement one correctly or to assess the correctness of an existing implementation.

% While a lot of work has focussed on rev mode AD, due to its heavy use in fitting neural nets
% using first order optimization algorithms, fwd mode AD should not be ignored.
% For computing higher order derivatives, nested first order AD is currently the method of choice: that is,
% fwd mode within fwd mode or fwd mode within rev mode, seeing that rev mode cannot be nested within rev mode.
% Such higher order derivatives are required for applications ranging from Laplace approximations 
% (requiring $2^{nd}$ order), via Riemannian HMC/NUTS 
% (requiring $3^{rd}$ order) \cite{girolami2009riemannian}, to higher order optimization algorithms.
% Moreover, it was recently shown that even for applications where a square Jacobian needs to be calculated,
% fwd mode outperforms rev mode \cite{shaikhha2019efficient}.
% Most importantly, however, we believe that it is instructive to consider the 
% semantics and correctness of fwd mode AD before proceeding to rev mode,
% as the former shares many of the challenges of the latter without the added,
% but orthogonal, complexity of non-local control flow. 
% \mv{Perhaps this paragraph can be removed if we also include rev AD.}

\vspace{-10pt}
\subsubsection{Formalization and correctness of automatic differentiation.}
Automatic differentiation systems like those implemented in TensorFlow \cite{abadi2016tensorflow} or Stan \cite{carpenter2015stan} form, in effect, the work-horse of modern machine learning and applied statistics.
They are the crucial low-level code on which all inference algorithms, and therefore modelling applications, depend.
A correct and efficient implementation of such a system is therefore of paramount importance.
However, proving correctness of existing implementations is challenging, as the written code is often highly optimized, for example to be run in parallel and on GPUs.
What is needed is a formalization of automatic differentiation, including a clear specification and correctness proof of various techniques used in practice.

Here, correctness means that the following diagram commutes, where $\sem{-}$ indicates some reasonable semantic interpretation.
\vspace{-11pt}
\[
	\xymatrix{
		 \textnormal{programs} \ar[rr]^{\sem{-}} \ar[d]_{\textnormal{syntactic differentiation}}
		 && \textnormal{differential geometry} \ar[d]^{\textnormal{semantic differentiation}} \\
		 \textnormal{programs}\ar[rr]^{\sem{-}}
		 && \textnormal{differential geometry}
	}
  \vspace{-7pt}\;
  \]
That is, the semantics of a program that has been syntactically differentiated using automatic differentiation equals the derivative of the semantics of the original program, where the derivative is taken in the usual semantic way familiar from calculus and differential geometry. At a minimum, correctness should be true of programs whose inputs and outputs are of first order type, like $\reals^n$ or some algebraic data type
holding reals like a type of lists of real vectors.


\vspace{-10pt}
\subsubsection{Related work and state-of-the-art.}
AD has a long history and has many implementations that cannot be discussed here in detail, hence the focus will be on particularly relevant references.
Various steps have been taken towards clear definitions of the algorithms involved. 
AD was first phrased in a functional setting and brought to the attention of a programming language audience in \cite{pearlmutter2008reverse}, also exposing the connection between rev mode AD and continuation-passing style.
Recently, Wang et al. demonstrated that rev mode AD can be clearly expressed using delimited continuations and that fwd mode AD can, similarly, be neatly phrased in terms of A-normal form transformations \cite{wang2018demystifying}.
Shaikhha et al. gave a particularly clean definition of fwd mode AD for a higher order language and showed how it is amenable to compiler optimizations \cite{shaikhha2019efficient}.
While independently discovered, differential $\lambda$-calculus \cite{ehrhard2003differential} appears closely related to fwd mode AD, though the connections have not been made precise.
Fong et al. noted that rev mode AD is a functor in a limited setting \cite{fong2019backprop}.
Similarly, but in the concrete context of a Haskell implementation, Elliot showed that both fwd and rev mode AD can be implemented as a functor \cite{elliott2018simple}.


Meanwhile, implementations are far ahead of the theoretical foundations.
For example, in Stan (and other systems), users routinely use AD-techniques on higher order functions like differential equation solvers to solve real-world problems, e.g. arising from pharmacological models used in early-stage clinical trials \cite{tsiros2019population}.
Similarly, AD-techniques are applied to recursive programs like recursive neural networks, which are used, for example, in natural language parsing \cite{socher2011parsing}.

Both fwd and rev AD techniques are currently lacking a semantic basis.
Indeed, while mathematical theories of differentiation accounting for higher order functions exist -- for example, diffeological spaces \cite{souriau1980groupes,iglesias2013diffeology} and synthetic differential geometry \cite{kock2006synthetic} -- they have not been connected to AD algorithms, let alone used to prove these algorithms correct. 
% Worse still, no satisfactory theory of differentiation which accounts for recursion exists.
While manifolds could suffice to prove correct AD on variant types, no such proof has been published.

Recently and independently of our work, a correctness proof of rev AD has emerged, relying on a syntactic argument using the 
linear substitution calculus, reducing terms until they have no higher order subterms and showing, by induction, the correctness of rev AD on first order programs  \cite{brunel2019backpropagation}.
We believe our proof methodology for showing correctness of AD is sufficiently different to be
independently of interest, as it relies on the use of a denotational semantics rather than syntactic methods.
Further, it applies uniformly to both fwd and rev AD as well as to a more expressive language with variant and inductive data types.


\vspace{-10pt}
\subsubsection{Our contributions.}
We have provided a semantic account of fwd and rev-mode AD. The main contributions of this work are the following novel constructions:
\begin{tightitemize}
\item an account of fwd-mode AD as a well-typed macro on a higher order language (\S \ref{sec:simple-language}) and a characterisation of its universal property, explaining why the definition is canonical  (Ex. \ref{ex:canonical-fwd});
\item a reasonable denotational semantics of this language (\S \ref{sec:semantics});
\item a definition and proof of correctness of fwd-mode AD with respect to this semantics (Th. \ref{thm:fwd-cor-basic});
\item an extension to variant and inductive types of fwd AD and its semantics (\S\ref{sec:extended-language}) as well as of the correctness proof  (\S \ref{sec:correctness}, Th. \ref{thm:fwd-cor-full});
\item an extension of all results to rev-AD (\S \ref{sec:rev-mode-short}, Th. \ref{thm:rev-cor-full}).
\end{tightitemize}


\vspace{-10pt}

==> polynomial-endofunctors.tex <==
\[
F ::= \id[\catC] \quad |\; \Delta(C)\quad |\; F(-)+F(-)\quad |\; F(-)\times F(-),
\]

==> rev-mode-k.tex <==
\section{$k$-Rev Mode}
\subsubsection{Rev AD as a structure preserving functor.}
To understand rev AD in the same framework, we can define a new macro
$\Dsynrevsymbol[k]$ on types and terms as the unique structure preserving functor
$\Syn\to\Syn$
such that 
\[
    \Dsynrev[k]{\reals} = \bProd{\reals}{(\reals\To\reals^k)}
\]
and
\[
\begin{array}{l}
    \Dsynrev[k]{\op(\trm_1,\ldots,\trm_n)} =\\
    \quad\pMatch{\Dsynrev[k]{\trm_1}}{\var_1}{\var_1'}{\ldots}\\
    \quad\pMatch{\Dsynrev[k]{\trm_n}}{\var_n}{\var_n'}{}\\
    \quad\quad\langle\op(\var_1,\ldots,\var_n),
    \fun{\var[2]:\reals}{}\var_1'(\op'(\var_1,1,\var_2,0,\ldots,\var_n,0) * \var[2])+\ldots\\
    \hspace{50pt} +
    \var_n'(\op'(\var_1,0,\ldots, \var_{n-1},0,\var_n,1) * \var[2])\rangle,
\end{array}
\]
where we assume that for each $n$-ary operation $\op$, we have some term 
\[
    \var_1,\var_1',\ldots,\var_n,\var_n':\reals\vdash 
\op'(\var_1,\var_1',\ldots,\var_n,\var_n'):\reals
\]
which calculates the (fwd)
derivative of $\op$.

To be explicit, we define $\Dsynrevsymbol[k]$ on other types and terms by
\[
\begin{array}{ll}
\Dsynrev[k]{\ty\To\ty[2]} = \Dsynrev[k]{\ty}\To\Dsynrev[k]{\ty[2]} \\
\Dsynrev[k]{\tProd{\ty_1}{\cdots}{\ty_n}} = \tProd{\Dsynrev[k]{\ty_1}}{\cdots}{\Dsynrev[k]{\ty_n}}\hspace{53pt}\, &\\
\Dsynrev[k]{\Variant{\Inj{\Cns_1}{\ty_1}\vor \ldots \vor\Inj{\Cns_n}{\ty_n}}} = 
\Variant{\Inj{\Cns_1}{\Dsynrev[k]{\ty_1}}\vor \ldots \vor\Inj{\Cns_n}{\Dsynrev[k]{\ty_n}}}\hspace{-40pt}\,&\\
\Dsynrev[k]{\List{\ty}} = \List{\Dsynrev[k]{\ty}}
\end{array}    
\]
and 
\[
\begin{array}{l}
\Dsynrev[k]{\var} = \var\\
\Dsynrev[k]{\fun \var    \trm} = \fun\var{\Dsynrev[k]{\trm}}\\
\Dsynrev[k]{\trm\, \trm[2] } = 
\Dsynrev[k]{\trm}\,\Dsynrev[k]{\trm[2]}\\
\Dsynrev[k]{\tTriple{\trm_1}{\dots}{\trm_n}} =\tTriple{\Dsynrev[k]{\trm_1}}{\dots}{\Dsynrev[k]{\trm_n}} \\
\Dsynrev[k]{{\tMatch{\trm}{\var_1,\dots,\var_n}{\trm[2]}}} =
\tMatch{\Dsynrev\trm}{\var_1,\dots,\var_n }{\Dsynrev[k]{\trm[2]}} \\
\Dsynrev[k]{\tInj\ty\Cns\trm} = \tInj{\Dsynrev[k]{\ty}}\Cns{\Dsynrev\trm}  \\
\Dsynrev[k]{\tNil} = \tNil\\
\Dsynrev[k]{\tCons{\trm}{\trm[2]}} = \tCons{\Dsynrev[k]{\trm}}{\Dsynrev[k]{\trm[2]}}\\
\Dsynrev[k]{\vMatch {\trm  }  {
    \Inj{\Cns_1}{\var_1}\To{\trm[2]_1}
\vor \cdots
\vor  \Inj{\Cns_n}{\var_n}\To{\trm[2]_n}
}} =\\
\qquad\vMatch {\Dsynrev\trm  }  {
    \Inj{\Cns_1}{\var_1}\To{\Dsynrev[k]{\trm[2]_1}}
\vor \cdots
\vor  \Inj{\Cns_n}{\var_n}\To{\Dsynrev[k]{\trm[2]_n}}
} \\
\Dsynrev[k]{\lFold{\var_1}{\var_2}{\trm}{\trm[2]}{\trm[3]}} =\\
\qquad\lFold{\var_1}{\var_2}{\Dsynrev\trm}{\Dsynrev[k]{\trm[2]}}{\Dsynrev[k]{\trm[3]}}
\end{array}
\]

\begin{theorem}
${\Dsynrevsymbol[k]}$ defines a structure preserving functor $\Syn\to\Syn$.
\end{theorem}

\subsubsection{Running reverse-mode AD.}
Then, observe that we can define, by induction of types, an embedding-retraction pair, 
embedding $\Dsyn[k]{\ty}$ into $\Dsynrev[k]{\ty}$ as the linear maps, for first order types
$\ty$.
We first specify the embedding
\begin{align*}
\var[3]:\Dsyn[k]{\ty}&\vdash\lamR[\ty][k]{\var[3]}: \Dsynrev[k]{\ty}\\
\var[3]:\Dsyn[k]{\reals} &\vdash \pMatch{\var[3]}{\var}{\var'}
{\tPair{\var}{\fun{\var[2]:\reals}{\var'*\var[2]}}}\\
\var[3]:\Dsyn[k]{\tProd{\ty_1}{\dots}{\ty_n}} &\vdash
\tMatch{\var[3]}{\tTriple{\var[3]_1}{\ldots}{\var[3]_n}}
{\tTriple{\lamR[\ty_1][k]{\var[3]_1}}{\ldots}{\lamR[\ty_n][k]{\var[3]_n}}}\\
\var[3]:\Dsyn[k]{\Variant{
    \Inj{\Cns_1}{\ty_1}
    \vor \ldots \vor
    \Inj{\Cns_n}{\ty_n}
  } } &\vdash 
  \vMatch {\trm  }  {
    \Inj{\Cns_1}{\var_1}\To{\Inj{\Cns_1}{\lamR[\ty_1][k]{\var_1}}}
\vor \cdots
\vor  \Inj{\Cns_n}{\var_n}\To{\Inj{\Cns_n}{\lamR[\ty_n][k]{\var_n}}}
}\\
\var[3]:\Dsyn[k]{\List{\ty}}&\vdash 
\lFold{\var_1}{\var_2}{\tCons{\lamR[\ty][k]{\var_1}}{\var_2}}{\var[3]}{\tNil}
\end{align*}
and then the retraction
\begin{align*}
\var[3]:\Dsynrev[k]{\ty}&\vdash\evR[\ty][k]{\var[3]}: \Dsyn[k]{\ty}\\
\var[3]:\Dsynrev[k]{\reals} & \vdash \pMatch{\var[3]}{\var}{\var'}{\tPair{\var}{\var'\, \underline{1}}}\\
\var[3]:\Dsynrev[k]{\tProd{\ty_1}{\dots}{\ty_n}} & \vdash 
\tMatch{\var[3]}{\tTriple{\var[3]_1}{\ldots}{\var[3]_n}}
{\tTriple{\evR[\ty_1]{\var[3]_1}}{\ldots}{\evR[\ty_n]{\var[3]_n}}}\\
\var[3]:\Dsynrev[k]{\Variant{
    \Inj{\Cns_1}{\ty_1}
    \vor \ldots \vor
    \Inj{\Cns_n}{\ty_n}
  } } &\vdash 
  \vMatch {\trm  }  {
    \Inj{\Cns_1}{\var_1}\To{\Inj{\Cns_1}{\evR[\ty_1][k]{\var_1}}}
\vor \cdots
\vor  \Inj{\Cns_n}{\var_n}\To{\Inj{\Cns_1}{\evR[\ty_n][k]{\var_n}}}
}\\
\var[3]:\Dsynrev[k]{\List{\ty}}&\vdash 
\lFold{\var_1}{\var_2}{\tCons{\evR[\ty][k]{\var_1}}{\var_2}}{\var[3]}{\tNil}.
\end{align*}
It is an easy exercise in induction to verify that these form an embedding-retraction pair.

\begin{lemma}
For all first order types $\ty$ (i.e. types not involving function types),
we have that $\evR[\ty][k]{\lamR[\ty][k]{\trm} }\beeq\trm$
(and that $\trm\beeq\lamR[\ty][k]{\evR[\ty][k]{\trm}}$ precisely when $\trm$ implements a
linear function -- but we should formalize what this means
before we can state it properly).
\end{lemma}

We run rev AD for a program $\trm\in\Syn(\ty,\ty[2])$
by running $\lamRsymbol[k]_{\ty};\Dsynrev[k]{\trm};\evRsymbol[k]_{\ty[2]}$.
This is, in fact, what systems like Stan and TensorFlow do in practice.
The idea is that $\Dsynrev[k]{\trm}$ is a higher order function that simultaneously runs
the forward pass and defines as a continuation the reverse pass of rev AD when applied
to $k$ cotangent vectors, that $\lamRsymbol[k]_{\ty}$ encodes tangent 
vectors as cotangent vectors so we can feed them into the higher order function
(in order to run the forward pass and define the reverse pass),
and that $\evRsymbol[k]_{\ty[2]}$ actually runs the reverse pass
by calling the continuation
and extracts $k$ tangent vectors
again.

\subsubsection{Correctness of reverse-mode AD.}
We use a variation on the gluing construction that we used for fwd AD.
Let $\Gl[\RR^k]$ be the full subcategory of $\id[\Diff]\downarrow \Diff(\RR^k,-)\times \Diff(\RR^k,-)$
on the subset inclusions.

In particular, one defines a binary logical relation $\semgl{\reals}^{r,k}=(\RR,\RR\times (\RR^k)^\RR, S^{r,k}_{\reals})$,
on the plots $\plots{\RR\times ((\RR^k)^\RR)}^{\RR^k}$, where
$$
S^{r,k}_{\reals}=
\left\{ \left(f,x\mapsto \sPair{f(x)}{y\mapsto \sTriple{\partial_1 f(x) * y}{\ldots}{\partial_k f(x) * y}}\right)\mid f\in\plots{\RR}^{\RR^k}\right\}
$$
that is 
$$
S^{r,k}_{\reals}=
\left\{ \left(f,\sPair{f(x)}{(\Dsemsymbol[k](f);\TtoD[,k]{\reals};\lamRsymbol[k]_{\reals})(e_1,\ldots, e_k)}\right)\mid f\in\plots{\RR}^{\RR^k}\right\}
$$
(For the standard basis $e_1,\ldots, e_k$ for $\RR^k$.)
We verify that $\sem{\cnst}\times \sem{\Dsynrev[k]{\cnst}}$, $\sem{\var+\var[2]}\times \sem{\Dsynrev[k]{\var +\var[2]}}$, $\sem{\var*\var[2]}\times \sem{\Dsynrev[k]{\var *\var[2]}}$ and $\sem{\sigmoid(\var)}\times \sem{\Dsynrev[k]{\sigmoid(\var)}}$
respect this logical relation.
It follows that this relation extends to a functor $\semgl{-}^{r,k}:\Syn\to\Gl[\RR^k]$ such that $\id\times \Dsynrevsymbol[k]$
factors over $\semgl{-}^{r,k}$.

In particular, we can calculate that $S^{r,k}_{\ty}$ for first order types $\ty$ represents the subset 
$$
\left\{ \left(f,\sPair{f(x)}{(\Dsemsymbol[k](f);\TtoD[,k]{\ty};\lamRsymbol[k]_{\ty})(e_1,\ldots, e_k)}\right)\mid f\in\plots{\sem{\ty}}^{\RR^k}\right\}.
$$
Because $\Dsynrev[k]{\trm}$ respects this logical relation for $\var:\ty\vdash \trm:\ty[2]$, it follows that for all smooth $f:\RR^k\to \sem{\ty}$, we have that 
$$
(\Dsemsymbol[k](f);\TtoD[,k]{\ty};\lamRsymbol[k]_{\ty};\Dsynrev[k]{\trm};\evR[k]{\ty[2]})(e_1,\ldots, e_k) = \Dsem[k]{f;\sem{\trm}}(e_1,\ldots,e_k).
$$

Recall the following well-known lemma.
\begin{lemma}\label{lem:partial-derivatives-2}
A smooth function $g: \Dsem[k]{M}\to \Dsem[k]{N}$ is of the form 
$\Dsem[k]{h}$ if for all smooth $f:\RR^k\to M$, we have that
$(\Dsem[k]{f};g)(e_1,\ldots,e_k)=\Dsem[k]{f;h}(e_1,\ldots,e_k)$.
\end{lemma}

Therefore, it follows that
$$
\TtoD[,k]{\ty};\lamRsymbol[k]_{\ty};\Dsynrev[k]{\trm};\evR[k]{\ty[2]} = \Dsem[k]{f;\sem{\trm}}.
$$

We have obtained the following correctness theorem.
\begin{theorem}[Semantic correctness of ${\Dsynrevsymbol[k]}$]
    \label{thm:rev-cor-full}
    For any ground $\ty$, any first order context $\Gamma$
    and any term $\Gamma\vdash\trm:\ty$,
    syntactic translation $\trm\mapsto \evR[{\ty}][k]{\subst{\Dsynrev[k]{\trm}}{\sfor{\var}{\lamR[\Gamma][k]{\var[3]}}}}$ coincides with the tangent bundle functor, modulo these canonical isomorphisms:
    \[\xymatrix{
        \sem{\Dsyn[k]\Gamma} \ar[rrr]^{\sem{\lamRsymbol[k]_{\Gamma};\Dsynrev[k]{\trm};\evRsymbol[k]_{\ty}}}  \ar[d]_{\DtoT[,k]{\Gamma}}^\cong
        &&&\sem{\Dsyn[k] \ty}\ar[d]^{\DtoT[,k]{\ty}}_\cong
        \\
        \Dsem[k]{\sem\Gamma}\ar[rrr]_{\Dsem[k]{\sem \trm}}
        &&&\Dsem[k]{\sem \ty}
        }\]
\end{theorem}

==> rev-mode.tex <==
\section{Rev Mode}
\subsubsection{Rev AD as a structure preserving functor.}
To understand rev AD in the same framework, we can define a new macro
$\Dsynrevsymbol$ on types and terms as the unique structure preserving functor
$\Syn\to\Syn$
such that 
\[
    \Dsynrev{\reals} = \bProd{\reals}{(\reals\To\reals)}
\]
and
\[
\begin{array}{l}
    \Dsynrev{\op(\trm_1,\ldots,\trm_n)} =\\
    \quad\pMatch{\Dsynrev{\trm_1}}{\var_1}{\var_1'}{\ldots}\\
    \quad\pMatch{\Dsynrev{\trm_n}}{\var_n}{\var_n'}{}\\
    \quad\quad\langle\op(\var_1,\ldots,\var_n),
    \fun{\var[2]:\reals}{}\var_1'(\op'(\var_1,1,\var_2,0,\ldots,\var_n,0) * \var[2])+\ldots\\
    \hspace{50pt} +
    \var_n'(\op'(\var_1,0,\ldots, \var_{n-1},0,\var_n,1) * \var[2])\rangle,
\end{array}
\]
where we assume that for each $n$-ary operation $\op$, we have some term 
\[
    \var_1,\var_1',\ldots,\var_n,\var_n':\reals\vdash 
\op'(\var_1,\var_1',\ldots,\var_n,\var_n'):\reals
\]
which calculates the (fwd)
derivative of $\op$.

To be explicit, we define $\Dsynrevsymbol$ on other types and terms by
\[
\begin{array}{ll}
\Dsynrev{\ty\To\ty[2]} = \Dsynrev{\ty}\To\Dsynrev{\ty[2]} \\
\Dsynrev{\tProd{\ty_1}{\cdots}{\ty_n}} = \tProd{\Dsynrev{\ty_1}}{\cdots}{\Dsynrev{\ty_n}}\hspace{53pt}\, &\\
\Dsynrev{\Variant{\Inj{\Cns_1}{\ty_1}\vor \ldots \vor\Inj{\Cns_n}{\ty_n}}} = 
\Variant{\Inj{\Cns_1}{\Dsynrev{\ty_1}}\vor \ldots \vor\Inj{\Cns_n}{\Dsynrev{\ty_n}}}\hspace{-40pt}\,&\\
\Dsynrev{\List{\ty}} = \List{\Dsynrev{\ty}}\\
\Dsynrev{\Tree{\ty}} = \Tree{\Dsynrev{\ty}}
\end{array}    
\]
and 
\[
\begin{array}{l}
\Dsynrev{\var} = \var\\
\Dsynrev{\fun \var    \trm} = \fun\var{\Dsynrev{\trm}}\\
\Dsynrev{\trm\, \trm[2] } = 
\Dsynrev{\trm}\,\Dsynrev{\trm[2]}\\
\Dsynrev{\tTriple{\trm_1}{\dots}{\trm_n}} =\tTriple{\Dsynrev{\trm_1}}{\dots}{\Dsynrev{\trm_n}} \\
\Dsynrev{{\tMatch{\trm}{\var_1,\dots,\var_n}{\trm[2]}}} =
\tMatch{\Dsynrev\trm}{\var_1,\dots,\var_n }{\Dsynrev{\trm[2]}} \\
\Dsynrev{\tInj\ty\Cns\trm} = \tInj{\Dsynrev{\ty}}\Cns{\Dsynrev\trm}  \\
\Dsynrev{\tNil} = \tNil\\
\Dsynrev{\tCons{\trm}{\trm[2]}} = \tCons{\Dsynrev{\trm}}{\Dsynrev{\trm[2]}}\\
\Dsynrev{\tLeaf\trm} = \tLeaf{\Dsynrev{\trm}}\\
\Dsynrev{\tNode\trm{\trm[2]}{\trm[3]}} = \tNode{\Dsynrev{\trm}}{\Dsynrev{\trm[2]}}{\Dsynrev{\trm[3]}}\\
\Dsynrev{\vMatch {\trm  }  {
    \Inj{\Cns_1}{\var_1}\To{\trm[2]_1}
\vor \cdots
\vor  \Inj{\Cns_n}{\var_n}\To{\trm[2]_n}
}} =\\
\qquad\vMatch {\Dsynrev\trm  }  {
    \Inj{\Cns_1}{\var_1}\To{\Dsynrev{\trm[2]_1}}
\vor \cdots
\vor  \Inj{\Cns_n}{\var_n}\To{\Dsynrev{\trm[2]_n}}
} \\
\Dsynrev{\lFold{\var_1}{\var_2}{\trm}{\trm[2]}{\trm[3]}} =\\
\qquad\lFold{\var_1}{\var_2}{\Dsynrev\trm}{\Dsynrev{\trm[2]}}{\Dsynrev{\trm[3]}}
\\
\Dsynrev{\tFold{\var_1}{\var_2}{\var_3}{\trm}{\trm[2]}{\var[2]}{\trm[3]}} =\\
\qquad\tFold{\var_1}{\var_2}{\var_3}{\Dsynrev\trm}{\Dsynrev{\trm[2]}}{\var[2]}{\Dsynrev{\trm[3]}} 
\end{array}
\]

\begin{theorem}
$\Dsynrevsymbol$ defines a structure preserving functor $\Syn\to\Syn$.
\end{theorem}

\subsubsection{Running reverse-mode AD.}
Then, observe that we can define, by induction of types, an embedding-retraction pair, 
embedding $\Dsyn{\ty}$ into $\Dsynrev{\ty}$ as the linear maps, for first order types
$\ty$.
We first specify the embedding
\begin{align*}
\var[3]:\Dsyn{\ty}&\vdash\lamR[\ty]{\var[3]}: \Dsynrev{\ty}\\
\var[3]:\Dsyn{\reals} &\vdash \pMatch{\var[3]}{\var}{\var'}
{\tPair{\var}{\fun{\var[2]:\reals}{\var'*\var[2]}}}\\
\var[3]:\Dsyn{\tProd{\ty_1}{\dots}{\ty_n}} &\vdash
\tMatch{\var[3]}{\tTriple{\var[3]_1}{\ldots}{\var[3]_n}}
{\tTriple{\lamR[\ty_1]{\var[3]_1}}{\ldots}{\lamR[\ty_n]{\var[3]_n}}}\\
\var[3]:\Dsyn{\Variant{
    \Inj{\Cns_1}{\ty_1}
    \vor \ldots \vor
    \Inj{\Cns_n}{\ty_n}
  } } &\vdash 
  \vMatch {\trm  }  {
    \Inj{\Cns_1}{\var_1}\To{\Inj{\Cns_1}{\lamR[\ty_1]{\var_1}}}
\vor \cdots
\vor  \Inj{\Cns_n}{\var_n}\To{\Inj{\Cns_n}{\lamR[\ty_n]{\var_n}}}
}\\
\var[3]:\Dsyn{\List{\ty}}&\vdash 
\lFold{\var_1}{\var_2}{\tCons{\lamR[\ty]{\var_1}}{\var_2}}{\var[3]}{\tNil}\\
\var[3]:\Dsyn{\Tree{\ty}}&\vdash 
\tFold{\var_1}{\var_2}{\var_3}{\tNode{\var_1}{\lamR[\ty]{\var_2}}
{\var_3}}{\var[3]}{\var[2]}{\tLeaf{\lamR[\ty]{\var[2]}}}.
\end{align*}
and then the retraction
\begin{align*}
\var[3]:\Dsynrev{\ty}&\vdash\evR[\ty]{\var[3]}: \Dsyn{\ty}\\
\var[3]:\Dsynrev{\reals} & \vdash \pMatch{\var[3]}{\var}{\var'}{\tPair{\var}{\var'\, \underline{1}}}\\
\var[3]:\Dsynrev{\tProd{\ty_1}{\dots}{\ty_n}} & \vdash 
\tMatch{\var[3]}{\tTriple{\var[3]_1}{\ldots}{\var[3]_n}}
{\tTriple{\evR[\ty_1]{\var[3]_1}}{\ldots}{\evR[\ty_n]{\var[3]_n}}}\\
\var[3]:\Dsynrev{\Variant{
    \Inj{\Cns_1}{\ty_1}
    \vor \ldots \vor
    \Inj{\Cns_n}{\ty_n}
  } } &\vdash 
  \vMatch {\trm  }  {
    \Inj{\Cns_1}{\var_1}\To{\Inj{\Cns_1}{\evR[\ty_1]{\var_1}}}
\vor \cdots
\vor  \Inj{\Cns_n}{\var_n}\To{\Inj{\Cns_1}{\evR[\ty_n]{\var_n}}}
}\\
\var[3]:\Dsynrev{\List{\ty}}&\vdash 
\lFold{\var_1}{\var_2}{\tCons{\evR[\ty]{\var_1}}{\var_2}}{\var[3]}{\tNil}\\
\var[3]:\Dsynrev{\Tree{\ty}}&\vdash 
\tFold{\var_1}{\var_2}{\var_3}{\tNode{\var_1}{\evR[\ty]{\var_2}}{\var_3}}{\var[3]}{\var[2]}{\tLeaf{\evR[\ty]{\var[2]}}}.
\end{align*}
It is an easy exercise in induction to verify that these form an embedding-retraction pair.

\begin{lemma}
For all first order types $\ty$ (i.e. types not involving function types),
we have that $\evR[\ty]{\lamR[\ty]{\trm} }\beeq\trm$
(and that $\trm\beeq\lamR[\ty]{\evR[\ty]{\trm}}$ precisely when $\trm$ implements a
linear function -- but we should formalize what this means
before we can state it properly).
\end{lemma}

We run rev AD for a program $\trm\in\Syn(\ty,\ty[2])$
by running $\lamRsymbol_{\ty};\Dsynrev{\trm};\evRsymbol_{\ty[2]}$.
This is, in fact, what systems like Stan and TensorFlow do in practice.
The idea is that $\Dsynrev{\trm}$ is a higher order function that simultaneously runs
the forward pass and defines as a continuation the reverse pass of rev AD when applied
to a cotangent vector, that $\lamRsymbol_{\ty}$ encodes a tangent 
vector as a cotangent vector so we can feed it into the higher order function
(in order to run the forward pass and define the reverse pass),
and that $\evRsymbol_{\ty[2]}$ actually runs the reverse pass
by calling the continuation
and extracts a tangent vector
again, so that we end up with a vector of numbers rather than a vector of functions.

\subsubsection{Semantics of reverse-mode AD.}
Note: we don't even seem to need these definitions, but it is how I think about these 
things.
In a way, we'd want to mirror the cotangent bundle construction in our type system, 
which we cannot quite do as we don't have linear function spaces, so we don't get an isomorphism
with the forward derivative, but an embedding-retraction pair instead, which seems good enough.
Perhaps the cotangent bundle is a red herring though as it does not seem to be needed.

Recall that for every manifold $M$, we have a definition of the cotangent bundle 
$\Dsemrev{M}=\sum_{x\in M}(\Dsemsymbol_x(M)\multimap \RR)$.
%which we can also apply
%to functions $f:M\to N$ by
%$\Dsemrevsymbol_x(f): \Dsemrevsymbol_{f(x)}N\to \Dsemrevsymbol_x M$;
%$\Dsemrevsymbol_x(f)(\xi)= \Dsemsymbol_x(f);\xi$.
%We also define $\Dsemrev{f}:f^*\Dsemrev{N}\to \Dsemrev{M} \to \Sigma_f\Dsemrev{M}$ by
%$\Dsemrev{f}(x,\xi)=(f(x), \Dsemsymbol_x(f);\xi)$.

We can now define (in $\Diff$) an embedding-retraction pair
\begin{align*}
\TtoDrev{\ty}:\Dsemrev{\sem{\ty}}&\to \sem{\Dsynrev{\ty}}\\
\DtoTrev{\ty}:\sem{\Dsynrev{\ty}}&\to \Dsemrev{\sem{\ty}}
\end{align*}
by induction on types, where $\TtoDrev{\ty};\DtoTrev{\ty}=\id$ and
$(\DtoTrev{\ty};\TtoDrev{\ty})(\eta)=\eta$ whenever $\eta$ defines a linear function.
These follow automatically
from $\evRsymbol$ and $\lamRsymbol$
if we note we have canonical isomorphisms (defined by induction):
\begin{align*}
\DsemtoDsemrev{\ty}:\Dsem{\sem{\ty}}&\to \Dsemrev{\sem{\ty}} \\
\DsemrevtoDsem{\ty}:\Dsemrev{\sem{\ty}}&\to \Dsem{\sem{\ty}} \\
\end{align*}
because of our canonical choice of coordinates on $\RR$.
Indeed, we can define
\begin{align*}
\TtoDrev{\ty}&=\DsemrevtoDsem{\ty};\TtoD{\ty};\sem{\lamRsymbol_{\ty}}\\
\DtoTrev{\ty}&=\sem{\evRsymbol_{\ty}};\DtoT{\ty};\DsemtoDsemrev{\ty}.
\end{align*}
Alternatively, we can define these maps more directly by noting that
\[
\Dsemrev{\sem{\reals}}=\RR \times (\RR\multimap \RR)\subseteq \RR\times (\RR\Rightarrow\RR)=\sem{\Dsynrev{\reals}}    
\]
which has the obvious retraction with sends $(x, f)$ to $(x, y\mapsto f(1) * y)$,
thus defining $\TtoDrev{\reals}$ and $\DtoTrev{\reals}$.
This generalizes from $\reals$ to arbitrary types $\ty$ by noting that both $\Dsemrevsymbol$ and $\Dsynrevsymbol$ 
preserve all type formers through canonical isomorphisms.

We can now observe that for $\trm\in\Syn(\ty,\ty[2])$,
$\Dsynrev{\trm}\in\Syn(\Dsynrev{\ty}.\Dsynrev{\ty[2]})$
and so $\TtoDrev{\ty};\sem{\Dsynrev{\trm}};\DtoTrev{\ty[2]}\in\Diff(\Dsemrev{\sem{\ty}},\Dsemrev{\sem{\ty[2]}})$.
What is a bit strange about this is that the morphisms in the fibre seem to be going in the wrong direction
for the cotangent bundle.
This is a mystery that I'd like to fully understand before we write a paper.
It has something to do with the fact that we have a canonical choice of coordinates because
we are working in the type hierarchy generated by $\RR$, which means that we have a canonical
isomorphism between tangent and cotangent, turning cotangent into a covariant functor as well.

\subsubsection{Correctness of reverse-mode AD.}
We use a variation on the gluing construction that we used for fwd AD.
Let $\Gl$ again be the full subcategory of $\id[\Diff]\downarrow \sem{\Dsynrev{-}}^\RR$
on the strong monos.

We now define an object $\glDrev(\reals)$ of $\Gl$ by
\begin{align*}
    m_{\glDrev(\reals)}:\RR^{\RR} \hookrightarrow &(\RR\times(\RR\Rightarrow \RR))^{\RR} =
    \sem{\Dsynrev{\reals}}^\RR\\
    f \mapsto & \left(x\mapsto \sPair{f(x)}{y\mapsto f'(x) * y}\right).
\end{align*}
We now calculate the following, which works for exactly the same reasons it did for 
fwd AD.
\begin{lemma}
Assuming that for each $n$-ary operation $\op$, 
$\sem{\op'}=\DtoT{\reals^n};\sem{\op}'$, we have
that
$\sem{\Dsynrev{\op}}^\RR$ restricts to a morphism
$\glDrev(\reals)^n\to\glDrev(\reals)$.
\end{lemma}
\begin{proof}
We compute 
\begin{align*}
&\sem{\Dsynrev{\op}}^\RR(x\mapsto \sTuple{f_1(x),y\mapsto f_1'(x)*y),\ldots,x\mapsto (f_n(x),
 y\mapsto f_n'(x)*y)}=\\
&\sTuple{x\mapsto (f_1(x),y\mapsto f_1'(x)*y),\ldots,x\mapsto (f_n(x),
 y\mapsto f_n'(x)*y)};\sem{\Dsynrev{\op}}^\RR=\\
 &x\mapsto \big(\sem{\op}(f_1(x),\ldots, f_n(x), y\mapsto 
 f_1'(x)*(\sem{\op'}(f_1(x),1,f_2(x),0,\ldots, f_n(x), 0)* y) + \ldots \\
 &+
 f_n'(x)*(\sem{\op'}(f_1(x),0,\ldots, f_{n-1}(x),0,\ldots, f_n(x), 1)*y)
 \big)=\\
 &
 x\mapsto \big(\sem{\op}(f_1(x),\ldots, f_n(x), y\mapsto 
 f_1'(x)*(\sem{\op}'(f_1(x),\ldots, f_n(x),1,0,\ldots, 0)* y) + \ldots\\
 & +
 f_n'(x)*(\sem{\op}'(f_1(x),\ldots, f_n(x), 0,\ldots, 0, 1)*y)
 \big)=\\
 &
 x\mapsto \big(\sem{\op}(f_1(x),\ldots, f_n(x), y\mapsto 
 (f_1'(x)*\sem{\op}'(f_1(x),\ldots, f_n(x),1,0,\ldots, 0) + \ldots\\
 & +
 f_n'(x)*\sem{\op}'(f_1(x),\ldots, f_n(x), 0,\ldots, 0, 1)) * y\big)=\\
 &
 x\mapsto \sPair{\sem{\op}(f_1(x),\ldots, f_n(x)}{ y\mapsto 
( \sTuple{f_1,\ldots,f_n};\sem{\op})'(x) * y}=\\
&
x\mapsto \sPair{(\sTuple{f_1,\ldots,f_n};\sem{\op})(x)}{ y\mapsto 
( \sTuple{f_1,\ldots,f_n};\sem{\op})'(x) * y}.
\end{align*}
\qed
\end{proof}
This lets us conclude the following.

\begin{lemma}
$\glDrev$ extends to a unique structure preserving functor $\Syn\to\Gl$ such that
$\glDrev;\projsyn=\Dsynrevsymbol$.
\end{lemma}
We can calculate that, for first order types $\ty$,
$\glDrev(\ty)=\sPair{\Dsynrev{\ty}}{m_{\glDrev(\ty)}}$,
where $m_{\glDrev(\ty)}$ represents the subset of $\sem{\Dsynrev{\ty}}^\RR$ consisting
of morphisms of the form  $\Delta_\RR;\Dsem{f};\TtoD{\ty};\sem{\lamRsymbol_{\ty}}$ for some
$f\in\sem{\ty}^\RR$.

Let us observe that $\Dsynrevsymbol=\glDrev;\projsyn$ implies that
for all $\trm\in\Syn(\ty,\ty[2])$ between first order types, we have that
$\sem{\Dsynrev{\trm}}^\RR$ restricts to a map
$m_{\glDrev(\ty)}\to m_{\glDrev(\ty[2])}$.
Take some smooth curve $\gamma: \RR\to \sem{\ty}$.
Then, note that $\Delta_{\RR};\Dsem{\gamma};\TtoD{\ty};\sem{\lamRsymbol_{\ty}}: \RR\to \sem{\Dsynrev{\ty}}$
is an element of $m_{\glDrev(\ty)}$.
Therefore, we get that $\sem{\Dsynrev{\trm}}^\RR(\Delta_{\RR};\Dsem{\gamma};\TtoD{\ty};\sem{\lamRsymbol_{\ty}})=
\Delta_{\RR};\Dsem{\gamma};\TtoD{\ty};\sem{\lamRsymbol_{\ty}};\sem{\Dsynrev{\trm}}$
is an element of $m_{\glDrev(\ty[2])}$ as well.
That is, it is of the form $\Delta_\RR;\Dsem{f};\TtoD{\ty[2]};\sem{\lamRsymbol_{\ty[2]}}$.
A quick calculation shows that $f=\gamma;\sem{\trm}$, so we obtain that 
$\Delta_{\RR};\Dsem{\gamma};\TtoD{\ty};\sem{\lamRsymbol_{\ty}}; \sem{\Dsynrev{\trm}}=
\Delta_\RR;\Dsem{\gamma;\sem{\trm}};\TtoD{\ty[2]};\sem{\lamRsymbol_{\ty[2]}}$
or, equivalently,\\ $\Dsem{\gamma};\TtoD{\ty};\sem{\lamRsymbol_{\ty}}; \sem{\Dsynrev{\trm}};\sem{\evRsymbol_{\ty[2]}};\DtoT{\ty[2]}
=\Dsem{\gamma;\sem{\trm}}$
for all smooth curves $\gamma: \reals\to \sem{\ty}$.
Recall the following well-known lemma.
\begin{lemma}\label{lem:partial-derivatives-2}
A smooth function $f: \Dsem{M}\to \Dsem{N}$ is of the form 
$\Dsem{g}$ if for all smooth curves $\gamma:\RR\to M$, we have that
$\Dsem{\gamma};f=\Dsem{\gamma;g}$.
\end{lemma}
Therefore, it follows that $\TtoD{\ty};\sem{\lamRsymbol_{\ty}}; \sem{\Dsynrev{\trm}};\sem{\evRsymbol_{\ty[2]}};\DtoT{\ty[2]}
=\Dsem{\sem{\trm}}$.

This lets us conclude correctness of $\Dsynrevsymbol$ in the following
sense.
\begin{theorem}[Semantic correctness of $\Dsynrevsymbol$ for higher order programs]
    \label{thm:revsemcorrectness2}
    For any term $\var:\ty\vdash \trm:\ty[2]$, where $\ty,\ty[2]$ do not involve function types, we have
    \[
    \TtoD{\ty};\sem{\lamRsymbol_{\ty};\Dsynrev{\trm};\evRsymbol_{\ty[2]}}
      = \Dsem{\sem{\trm}};\TtoD{\ty[2]}.
    \]
\end{theorem}
